Solving the Discrete Euler-Arnold Equations for the Generalized Rigid Body Motion

We propose three iterative methods for solving the Moser-Veselov equation, which arises in the discretization of the Euler-Arnold differential equations governing the motion of a generalized rigid body. We start by formulating the problem as an optimization problem with orthogonal constraints and proving that the objective function is convex. Then, using techniques from optimization on Riemannian manifolds, the three feasible algorithms are designed. The first one splits the orthogonal constraints using the Bregman method, whereas the other two methods are of the steepest-descent type. The second method uses the Cayley-transform to preserve the constraints and a Barzilai-Borwein step size, while the third one involves geodesics, with the step size computed by Armijo's rule. Finally, a set of numerical experiments are carried out to compare the performance of the proposed algorithms, suggesting that the first algorithm has the best performance in terms of accuracy and number of iterations. An essential advantage of these iterative methods is that they work even when the conditions for applicability of the direct methods available in the literature are not satisfied.

==> files/closedForm.tex <==
\section{Closed-Form Solutions}
In several problems, it required a solution the problem of \eqref{eq:fobj_1} as fast as possible. For that purpose, in this section we exploit the cases in which we can solve it in close problems.

\subsection{The case in which ${X}\in\mathcal{SO}(2)$}
For this case, one has
\begin{equation}
    {J} =
    \begin{bmatrix}
        j_1 & j_2 \\ j_2 & j_3
    \end{bmatrix}; \ \
    \mathbf{M} =
    \begin{bmatrix}
        0 & m_1 \\ -m1 & 0
    \end{bmatrix}; \ \ \text{and} \ \
    \mathbf{X} =
    \begin{bmatrix}
        c\theta & -s\theta \\ s\theta & c\theta
    \end{bmatrix},
\end{equation}
in which $s\theta$ and $c\theta$ denotes the $\text{sin}(\theta)$ and $\text{cos}(\theta)$ respectively. By expanding \eqref{simp_of} using these matrices:
\begin{equation}
    \mathcal{F}(\mathbf{X}) = \kappa_1 c\theta^2 + \kappa_2 s\theta^2 + \kappa_3 s\theta + \kappa_4,
\end{equation}
in which:
\begin{align}
    \kappa_1 & \ = - 2j_1^2 - 4j_2^2 - 2j_3^2; \\
    \kappa_2 & \ = - 4j_2^2 + 4j_1 j_3; \\
    \kappa_3 & \ = - 4j_1 m_1 - 4j_3 m_1;\ \  \text{and} \\
    \kappa_4 & \ = 2 j_1^2 + 4 j_2^2 + 2 j_3^2 + 2 m_1^2.
\end{align}

Now, by replacing $c\theta^2 = 1- s\theta$ (trigonometric relation), we can easily get a the polynomial equation:
\begin{equation}
    \mathcal{F}(\mathbf{X}) = (\kappa_2-\kappa_1) s\theta^2 + \kappa_3 s\theta + (\kappa_1 + \kappa_4).
\end{equation}

From the above derivations, a simple conclusion can be drawn.

\begin{theorem}
For the case of the $\mathbf{X}\in\mathcal{SO}(2)$, we have two solutions to the problem of \eqref{eq:fobj_1} which are given by
\begin{equation}
    s\theta = \frac{m_1}{j_1 + j_3}\ \ \text{and} \ \
    c\theta = \pm \sqrt{1-\frac{m_1}{j_1 + j_3}}.
\end{equation}
\end{theorem}
